Understanding GNNs for Boolean Satisfiability through Approximation Algorithms

The paper deals with the interpretability of Graph Neural Networks in the context of Boolean Satisfiability. The goal is to demystify the internal workings of these models and provide insightful perspectives into their decision-making processes. This is done by uncovering connections to two approximation algorithms studied in the domain of Boolean Satisfiability: Belief Propagation and Semidefinite Programming Relaxations. Revealing these connections has empowered us to introduce a suite of impactful enhancements. The first significant enhancement is a curriculum training procedure, which incrementally increases the problem complexity in the training set, together with increasing the number of message passing iterations of the Graph Neural Network. We show that the curriculum, together with several other optimizations, reduces the training time by more than an order of magnitude compared to the baseline without the curriculum. Furthermore, we apply decimation and sampling of initial embeddings, which significantly increase the percentage of solved problems.

==> images/images/res_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
Problem type                                & \begin{tabular}[c]{@{}c@{}}\#SAT \\ problems\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ \#var\end{tabular} & \begin{tabular}[c]{@{}c@{}}First\\ pass\end{tabular} & \begin{tabular}[c]{@{}c@{}}Second\\ pass\end{tabular} & \begin{tabular}[c]{@{}c@{}}\#MP\\ iterations\end{tabular} & \#samples & Decimation & Solved   \\ \toprule
\multirow{3}{*}{\textbf{SR(40)}}            & \multirow{3}{*}{5000}                                     & \multirow{3}{*}{40}                                  & 4442                                                 & 274                                                   & \multirow{3}{*}{100}                                      & 16        & Yes        & 94 \%    \\
                                            &                                                           &                                                      & 3990                                                 & -                                                     &                                                           & 1         & No         & 80 \%    \\
                                            &                                                           &                                                      & 4457                                                 & -                                                     &                                                           & 32        & No         & 89.1 \%  \\ \toprule
\multirow{3}{*}{\textbf{Latin Squares 9x9}} & \multirow{3}{*}{200}                                      & \multirow{3}{*}{196.9}                               & 186                                                  & 14                                                    & \multirow{3}{*}{1000}                                     & 16        & Yes        & 100 \%   \\
                                            &                                                           &                                                      & 95                                                   & -                                                     &                                                           & 1         & No         & 47.5 \%  \\
                                            &                                                           &                                                      & 192                                                  & -                                                     &                                                           & 32        & No         & 96 \%    \\ \toprule
\multirow{3}{*}{\textbf{Latin Squares 8x8}} & \multirow{3}{*}{200}                                      & \multirow{3}{*}{133.5}                               & 196                                                  & 1                                                     & \multirow{3}{*}{1000}                                     & 16        & Yes        & 98.5 \%  \\
                                            &                                                           &                                                      & 113                                                  & -                                                     &                                                           & 1         & No         & 56.5 \%  \\
                                            &                                                           &                                                      & 197                                                  & -                                                     &                                                           & 32        & No         & 98.5 \%  \\ \toprule
\multirow{3}{*}{\textbf{Logical Circuits}}  & \multirow{3}{*}{344}                                      & \multirow{3}{*}{131.1}                               & 319                                                  & 0                                                     & \multirow{3}{*}{1000}                                     & 16        & Yes        & 92.7 \%  \\
                                            &                                                           &                                                      & 293                                                  & -                                                     &                                                           & 1         & No         & 85.2 \%  \\
                                            &                                                           &                                                      & 319                                                  & -                                                     &                                                           & 32        & No         & 92.73 \% \\ \toprule
\multirow{3}{*}{\textbf{Sudoku 9x9}}        & \multirow{3}{*}{200}                                      & \multirow{3}{*}{245.6}                               & 92                                                   & 11                                                    & \multirow{3}{*}{1000}                                     & 16        & Yes        & 51.5 \%  \\
                                            &                                                           &                                                      & 35                                                   & -                                                     &                                                           & 1         & No         & 17.5 \%  \\
                                            &                                                           &                                                      & 94                                                   & -                                                     &                                                           & 32        & No         & 47 \%    \\ \toprule
\end{tabular}}
\caption{Improvements obtained due to the sampling and decimation procedure. We test how many satisfiable problems could be solved with the model. \textbf{SR(40)} is the test set with random problems; the other prolems are describe in Appendix \ref{appendix:structured}. For each problem type, we include the \textbf{average number of variables}. For larger problems, we run the model for more MP iterations. When decimation is used, we count the number of problems solved during the \textbf{first and the second pass} separately. \textbf{\#samples} refers to the number of different initializations of literal embeddings.}\label{tab:res}
\end{table}

==> images/images/res_table2.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{\begin{tabular}{lcccccccc}
\toprule
Problem type                                & \begin{tabular}[c]{@{}c@{}}\#SAT \\ problems\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg. \\ \#var\end{tabular} & \begin{tabular}[c]{@{}c@{}}First \\ pass\end{tabular} & \begin{tabular}[c]{@{}c@{}}Second\\ pass\end{tabular} & \begin{tabular}[c]{@{}c@{}}\#MP \\ iterations\end{tabular} & \#samples & Decimation & Solved  \\ \midrule
\multirow{3}{*}{\textbf{SR(40)}}            & \multirow{2}{*}{5000}                                     & \multirow{2}{*}{40}                                   & 4442                                                  & 274                                                   & \multirow{2}{*}{100}                                       & 16        & Yes        & 94\%    \\
                                            &                                                           &                                                       & 3990                                                  & -                                                     &                                                            & 1         & No         & 80\%    \\ \midrule
\multirow{2}{*}{\textbf{Latin Squares 9x9}} & \multirow{2}{*}{200}                                      & \multirow{2}{*}{196.9}                                  & 186                                                   & 14                                                    & \multirow{2}{*}{1000}                                      & 16        & Yes        & 100 \%  \\
                                            &                                                           &                                                       & 95                                                    & -                                                     &                                                            & 1         & No         & 47.5\%  \\ \midrule
\multirow{2}{*}{\textbf{Latin Squares 8x8}} & \multirow{2}{*}{200}                                      & \multirow{2}{*}{133.5}                                  & 196                                                   & 1                                                     & \multirow{2}{*}{1000}                                      & 16        & Yes        & 98.5 \% \\
                                            &                                                           &                                                       & 113                                                   & -                                                     &                                                            & 1         & No         & 56.5 \% \\ \midrule
\multirow{2}{*}{\textbf{Logical Circuits}}  & \multirow{2}{*}{344}                                      & \multirow{2}{*}{131.1}                                   & 319                                                   & 0                                                     & \multirow{2}{*}{1000}                                      & 16        & Yes        & 92.7 \% \\
                                            &                                                           &                                                       & 293                                                   & -                                                     &                                                            & 1         & No         & 85.2 \% \\ \midrule
\multirow{2}{*}{\textbf{Sudoku 9x9}}        & \multirow{2}{*}{200}                                      & \multirow{2}{*}{245.6}                                  & 92                                                    & 11                                                    & \multirow{2}{*}{1000}                                      & 16        & Yes        & 51.5 \% \\
                                            &                                                           &                                                       & 35                                                    & -                                                     &                                                            & 1         & No         & 17.5 \% \\ \bottomrule
\end{tabular}}
\caption{This table shows improvements obtained due to the sampling and decimation procedure. We test how many satisfiable problems could be solved with the model. \textbf{SR(40)} is the test set with random problems; the other prolems are describe in Appendix \ref{appendix:structured}. For each problem type, we include the \textbf{average number of variables}. For larger problems, we run the model for more MP iterations. When decimation is used, we count the number of problems solved during the \textbf{first and the second pass} separately. \textbf{\#samples} refers to the number of different initializations of literal embeddings.}\label{tab:res}
\end{table}

==> images/res_table2.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{\begin{tabular}{lcccccccc}
\toprule
Problem type                                & \begin{tabular}[c]{@{}c@{}}\#SAT \\ problems\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg. \\ \#var\end{tabular} & \begin{tabular}[c]{@{}c@{}}First \\ pass\end{tabular} & \begin{tabular}[c]{@{}c@{}}Second\\ pass\end{tabular} & \begin{tabular}[c]{@{}c@{}}\#MP \\ iterations\end{tabular} & \#samples & Decimation & Solved  \\ \midrule
\multirow{3}{*}{\textbf{SR(40)}}            & \multirow{2}{*}{5000}                                     & \multirow{2}{*}{40}                                   & 4442                                                  & 274                                                   & \multirow{2}{*}{100}                                       & 16        & Yes        & 94\%    \\
                                            &                                                           &                                                       & 3990                                                  & -                                                     &                                                            & 1         & No         & 80\%    \\ \midrule
\multirow{2}{*}{\textbf{Latin Squares 9x9}} & \multirow{2}{*}{200}                                      & \multirow{2}{*}{196.9}                                  & 186                                                   & 14                                                    & \multirow{2}{*}{1000}                                      & 16        & Yes        & 100 \%  \\
                                            &                                                           &                                                       & 95                                                    & -                                                     &                                                            & 1         & No         & 47.5\%  \\ \midrule
\multirow{2}{*}{\textbf{Latin Squares 8x8}} & \multirow{2}{*}{200}                                      & \multirow{2}{*}{133.5}                                  & 196                                                   & 1                                                     & \multirow{2}{*}{1000}                                      & 16        & Yes        & 98.5 \% \\
                                            &                                                           &                                                       & 113                                                   & -                                                     &                                                            & 1         & No         & 56.5 \% \\ \midrule
\multirow{2}{*}{\textbf{Logical Circuits}}  & \multirow{2}{*}{344}                                      & \multirow{2}{*}{131.1}                                   & 319                                                   & 0                                                     & \multirow{2}{*}{1000}                                      & 16        & Yes        & 92.7 \% \\
                                            &                                                           &                                                       & 293                                                   & -                                                     &                                                            & 1         & No         & 85.2 \% \\ \midrule
\multirow{2}{*}{\textbf{Sudoku 9x9}}        & \multirow{2}{*}{200}                                      & \multirow{2}{*}{245.6}                                  & 92                                                    & 11                                                    & \multirow{2}{*}{1000}                                      & 16        & Yes        & 51.5 \% \\
                                            &                                                           &                                                       & 35                                                    & -                                                     &                                                            & 1         & No         & 17.5 \% \\ \bottomrule
\end{tabular}}
\caption{This table shows improvements obtained due to the sampling and decimation procedure. We test how many satisfiable problems could be solved with the model. \textbf{SR(40)} is the test set with random problems; the other prolems are describe in Appendix \ref{appendix:structured}. For each problem type, we include the \textbf{average number of variables}. For larger problems, we run the model for more MP iterations. When decimation is used, we count the number of problems solved during the \textbf{first and the second pass} separately. \textbf{\#samples} refers to the number of different initializations of literal embeddings.}\label{tab:res}
\end{table}

==> sections/reproducibility.tex <==
In the supplementary material, we provide a source code with a readme that allows to reproduce the results of our model presented in Figure \ref{fig:model_performance} and Table \ref{tab:res}. Results for NeuroSAT presented in Figure\ref{fig:model_performance} were obtained by running training scripts in the publically available implementaion of NeuroSAT available at this url:\url{https://github.com/ryanzhangfan/NeuroSAT/tree/master}.

==> sections/temp.tex <==
The quality of the obtained solution is largely dependent on the \emph{convergence threshold}, which determines when the optimization should stop. Empirically, as problems become more difficult to solve, a smaller threshold is needed to obtain a good quality solution. A smaller threshold, results in more steps that update the vectors being optimized. This observation motivates our training procedure.



The substantial improvement in training time, by orders of magnitude compared to the original NeuroSat, was not solely the result of introducing curriculum learning. It was also achieved through significant changes in model architecture and training hyperparameters.


Both models share core components, including message passing, LSTM updates, and voting. However, our implementation adds flexibility through incremental training and batch processing, enabling efficient adaptation to problems of varying sizes.
While the original NeuroSAT model employs layer-normalized LSTMs to update vector representations of literals and clauses, our implementation utilizes vanilla LSTM layers for the same purpose.


In terms of training, we follow an incremental approach with a maximum of 200 epochs, a learning rate of 2e-3 (using Adam optimizer), and a batch size of 128. During validation, we monitor accuracy and employ early stopping when a certain threshold is reached. This threshold may seem arbitrary but setting it between 60\% and 70\% aligns with our model's initial random guessing phase. Accuracy slightly above 50\% at the start might be attributed to insignificant fluctuations. Empirical study reveals that the most challenging and time-consuming part of learning is the phase transition between random guessing and maintaining accuracy above 55\%. Once the model achieves this accuracy level, it continues to improve steadily.

Even though the method we propose is applicable to a wide range of domains of combinatorial optimization, in this work, we focus on applications of GNN in the domain of boolean satisfiability, specifically on the end-to-end approaches. From the implementation point of view, the proposed method requires minimal changes to the GNN architecture and the training loop. We demonstrated it in the context of learning to predict the satisfiability status of a boolean formula from a single bit supervision.

We also show that we can replace the classifier layer, which produces votes for each literal, with a procedure that computes a clustering coefficient for these vectors and predicts the formula as satisfiable if this coefficient is above a certain threshold. With this procedure, we achieve the same accuracy as with the original classifier used for training. 





In our endeavor to reproduce the original NeuroSAT work, we encountered challenges as the authors only shared a version for a smaller dataset on their GitHub repository. Additionally, an alternative implementation in PyTorch, authored by a different individual, is also publicly available. 

To replicate the original experiment, we must rely on these resources and the descriptions provided in the paper. This process can be quite challenging, particularly when aiming to achieve results that surpass random guessing, as extensive training hours are often required before the model starts generating meaningful predictions. It is plausible that the authors of the original paper employed specific techniques or regularization methods that were not explicitly documented in their work, but it also created a space for an improvement. 

This has motivated our team to explore alternative approaches, investigate the model's capabilities in greater depth, and effort to provide a more comprehensive interpretation of its behavior. As a commitment to fostering reproducibility and future research, we will make our implementation publicly available, complete with detailed usage instructions, enabling other researchers to study the model with greater ease.


Our work is another contribution to the field where learned approaches are used in the context of problem solving algorithms. In our case the machine learning algorithm aims to predict satisfiability and even find solution end-to-end, but many previous work focused to use such algorithms only to guide the hand designed solver or select it from the predefined portfolio. In the context of SAT very popular is portfolio based selector SATzilla \cite{xu2008satzilla}, which chooses the best SAT solver online on per-instance basis. Similar to that \cite{scott2021machsmt} transferred that approach to the domain of SMT (Satisfiability Modulo Theories) with their MachSMT selector. Both those works as empirical hardness models and predict the best solver based on expertly selected and domain specific features.

Idea of encoding a mathematical expression as a graph for representation learning is also well studied, for example by \cite{wang2017premise} who used it for premise selection in automated proving.

Taking a more intricate approach, there is the concept of selecting a solving strategy tailored to a single solver. An illustrative example of this approach is presented in the work of \cite{balunovic2018learning}, which treats the task of solving SMT formulas as a tree search problem. Here, for each formula (from a set of unsolved formulas) at a given step a learned policy selects a suitable transformation to apply. Policy decisions are synthesized into a strategy in the form of a loop-free program with branches.
